Non-Semantic Evaluation of Image Forensics Tools: Methodology and Database

With the aim of evaluating image forensics tools, we propose a methodology to create forgeries traces, leaving intact the semantics of the image. Thus, the only forgery cues left are the specific alterations of one or several aspects of the image formation pipeline. This methodology creates automatically forged images that are challenging to detect for forensic tools and overcomes the problem of creating convincing semantic forgeries. Based on this methodology, we create the Trace database and conduct an evaluation of the main state-of-the-art image forensics tools.

==> old_table.tex <==
%This file was automatically generated. Manual changes will be erased if the file is regenerated
\begin{tabular}{llcccccc}
\toprule
&&&&Dataset\vspace{7pt}\\
&&Noise Level&CFA Grid&CFA Algorithm&JPEG Grid&JPEG Quality&Hybrid\\\midrule
\multirow{6}{*}{\rotatebox{90}{Noise-based}}&\multirow{2}{*}{Splicebuster~\cite{splicebuster2015}}&\noTableValue\tableScoreSeparator\sIoU{\tbest{0.073}} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.056} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.059} & \noTableValue\tableScoreSeparator\sIoU{0.063}\\
&&\gIoU{0.139}\tableScoreSeparator\lIoU{0.203} & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.097}\tableScoreSeparator\lIoU{0.149} & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.104}\tableScoreSeparator\lIoU{0.148} & \gIoU{0.112}\tableScoreSeparator\lIoU{0.157}\tableVerticalSeparator\\
&\multirow{2}{*}{Lyu~\cite{lyupan2013}}&\noTableValue\tableScoreSeparator\sIoU{0.035} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.035} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.035} & \noTableValue\tableScoreSeparator\sIoU{0.034}\\
&&\gIoU{0.046}\tableScoreSeparator\lIoU{0.096} & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.038}\tableScoreSeparator\lIoU{0.052} & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.037}\tableScoreSeparator\lIoU{0.050} & \gIoU{0.037}\tableScoreSeparator\lIoU{0.063}\tableVerticalSeparator\\
&\multirow{2}{*}{Mahdian~\cite{mahdian2009}}&\noTableValue\tableScoreSeparator\sIoU{0.036} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.033}\\
&&\gIoU{0.063}\tableScoreSeparator\lIoU{0.192} & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.044}\tableScoreSeparator\lIoU{0.098} & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.042}\tableScoreSeparator\lIoU{0.085} & \gIoU{0.049}\tableScoreSeparator\lIoU{0.106}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{6}{*}{\rotatebox{90}{CFA-based}}&\multirow{2}{*}{Bammey~\cite{bammey}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{\tbest{0.416}} & \noTableValue\tableScoreSeparator\sIoU{\tbest{0.303}} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.086}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \gIoU{\tbest{0.498}}\tableScoreSeparator\lIoU{\tbest{0.511}} & \gIoU{\tbest{0.359}}\tableScoreSeparator\lIoU{\tbest{0.380}} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.089}\tableScoreSeparator\lIoU{0.103}\tableVerticalSeparator\\
&\multirow{2}{*}{Shin~\cite{shin2017color}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.043} & \noTableValue\tableScoreSeparator\sIoU{0.042} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.034}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.054}\tableScoreSeparator\lIoU{0.058} & \gIoU{0.049}\tableScoreSeparator\lIoU{0.055} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.038}\tableScoreSeparator\lIoU{0.042}\tableVerticalSeparator\\
&\multirow{2}{*}{Choi~\cite{choi}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.032}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.033}\tableScoreSeparator\lIoU{0.035} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.034} & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.033}\tableScoreSeparator\lIoU{0.034}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{14}{*}{\rotatebox{90}{JPEG-based}}&\multirow{2}{*}{Zero~\cite{ZERO}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \bIoU{\tbest{0.718}}\tableScoreSeparator\sIoU{\tbest{0.718}} & \bIoU{\tbest{0.700}}\tableScoreSeparator\sIoU{\tbest{0.700}} & \bIoU{\tbest{0.602}}\tableScoreSeparator\sIoU{\tbest{0.602}}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{\tbest{0.718}}\tableScoreSeparator\lIoU{\tbest{0.718}} & \gIoU{\tbest{0.700}}\tableScoreSeparator\lIoU{\tbest{0.700}} & \gIoU{\tbest{0.602}}\tableScoreSeparator\lIoU{\tbest{0.602}}\tableVerticalSeparator\\
&\multirow{2}{*}{CAGI~\cite{CAGI}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.030}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.096}\tableScoreSeparator\lIoU{0.182} & \gIoU{0.097}\tableScoreSeparator\lIoU{0.187} & \gIoU{0.081}\tableScoreSeparator\lIoU{0.174}\tableVerticalSeparator\\
&\multirow{2}{*}{FDF-A~\cite{ADQ3}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.088} & \noTableValue\tableScoreSeparator\sIoU{0.091} & \noTableValue\tableScoreSeparator\sIoU{0.083}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.115}\tableScoreSeparator\lIoU{0.122} & \gIoU{0.118}\tableScoreSeparator\lIoU{0.124} & \gIoU{0.108}\tableScoreSeparator\lIoU{0.114}\tableVerticalSeparator\\
&\multirow{2}{*}{I-CDA~\cite{ADQ2}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.167} & \noTableValue\tableScoreSeparator\sIoU{0.160} & \noTableValue\tableScoreSeparator\sIoU{0.175}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.327}\tableScoreSeparator\lIoU{0.390} & \gIoU{0.317}\tableScoreSeparator\lIoU{0.378} & \gIoU{0.245}\tableScoreSeparator\lIoU{0.293}\tableVerticalSeparator\\
&\multirow{2}{*}{CDA~\cite{ADQ1}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.217} & \noTableValue\tableScoreSeparator\sIoU{0.218} & \noTableValue\tableScoreSeparator\sIoU{0.187}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.262}\tableScoreSeparator\lIoU{0.300} & \gIoU{0.260}\tableScoreSeparator\lIoU{0.297} & \gIoU{0.219}\tableScoreSeparator\lIoU{0.254}\tableVerticalSeparator\\
&\multirow{2}{*}{BAG~\cite{BLK}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.127} & \noTableValue\tableScoreSeparator\sIoU{0.126} & \noTableValue\tableScoreSeparator\sIoU{0.109}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.128}\tableScoreSeparator\lIoU{0.128} & \gIoU{0.126}\tableScoreSeparator\lIoU{0.126} & \gIoU{0.109}\tableScoreSeparator\lIoU{0.109}\tableVerticalSeparator\\
&\multirow{2}{*}{ELA~\cite{ELA}}&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.056}\tableScoreSeparator\lIoU{0.071} & \gIoU{0.060}\tableScoreSeparator\lIoU{0.079} & \gIoU{0.059}\tableScoreSeparator\lIoU{0.077}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{8}{*}{\rotatebox{90}{Generic tools}}&\multirow{2}{*}{Noiseprint~\cite{noiseprint}}&\bIoU{\tbest{0.108}}\tableScoreSeparator\sIoU{0.068} & \bIoU{0.034}\tableScoreSeparator\sIoU{0.033} & \bIoU{\tbest{0.068}}\tableScoreSeparator\sIoU{0.047} & \bIoU{0.042}\tableScoreSeparator\sIoU{0.034} & \bIoU{0.166}\tableScoreSeparator\sIoU{0.071} & \bIoU{0.127}\tableScoreSeparator\sIoU{0.065}\\
&&\gIoU{\tbest{0.152}}\tableScoreSeparator\lIoU{\tbest{0.217}} & \gIoU{0.039}\tableScoreSeparator\lIoU{0.054} & \gIoU{0.091}\tableScoreSeparator\lIoU{0.137} & \gIoU{0.047}\tableScoreSeparator\lIoU{0.071} & \gIoU{0.202}\tableScoreSeparator\lIoU{0.270} & \gIoU{0.159}\tableScoreSeparator\lIoU{0.217}\tableVerticalSeparator\\
&\multirow{2}{*}{ManTraNet~\cite{mantranet}}&\bIoU{0.059}\tableScoreSeparator\sIoU{0.050} & \bIoU{0.038}\tableScoreSeparator\sIoU{0.036} & \bIoU{0.087}\tableScoreSeparator\sIoU{0.062} & \bIoU{0.040}\tableScoreSeparator\sIoU{0.036} & \bIoU{0.142}\tableScoreSeparator\sIoU{0.082} & \bIoU{0.124}\tableScoreSeparator\sIoU{0.078}\\
&&\gIoU{0.067}\tableScoreSeparator\lIoU{0.088} & \gIoU{0.039}\tableScoreSeparator\lIoU{0.047} & \gIoU{0.089}\tableScoreSeparator\lIoU{0.129} & \gIoU{0.042}\tableScoreSeparator\lIoU{0.050} & \gIoU{0.162}\tableScoreSeparator\lIoU{0.214} & \gIoU{0.125}\tableScoreSeparator\lIoU{0.169}\tableVerticalSeparator\\
%&Self-Consistency~\cite{selfconsistency}&\bIoU{0.043}\tableScoreSeparator\sIoU{0.044} & \bIoU{0.034}\tableScoreSeparator\sIoU{0.035} & \bIoU{0.037}\tableScoreSeparator\sIoU{0.036} & \bIoU{0.035}\tableScoreSeparator\sIoU{0.034} & \bIoU{0.052}\tableScoreSeparator\sIoU{0.040} & \bIoU{0.041}\tableScoreSeparator\sIoU{0.039}\\
%&with DB-SCAN&\gIoU{0.067}\tableScoreSeparator\lIoU{0.099} & \gIoU{0.042}\tableScoreSeparator\lIoU{0.060} & \gIoU{0.047}\tableScoreSeparator\lIoU{0.069} & \gIoU{0.041}\tableScoreSeparator\lIoU{0.060} & \gIoU{0.055}\tableScoreSeparator\lIoU{0.088} & \gIoU{0.053}\tableScoreSeparator\lIoU{0.085}\tableVerticalSeparator\\
&\multirow{2}{*}{Self-Consistency~\cite{selfconsistency}}&\bIoU{0.042}\tableScoreSeparator\sIoU{0.041} & \bIoU{0.035}\tableScoreSeparator\sIoU{0.035} & \bIoU{0.037}\tableScoreSeparator\sIoU{0.035} & \bIoU{0.035}\tableScoreSeparator\sIoU{0.034} & \bIoU{0.048}\tableScoreSeparator\sIoU{0.037} & \bIoU{0.041}\tableScoreSeparator\sIoU{0.038}\\
&&\gIoU{0.064}\tableScoreSeparator\lIoU{0.092} & \gIoU{0.041}\tableScoreSeparator\lIoU{0.059} & \gIoU{0.046}\tableScoreSeparator\lIoU{0.066} & \gIoU{0.040}\tableScoreSeparator\lIoU{0.057} & \gIoU{0.054}\tableScoreSeparator\lIoU{0.082} & \gIoU{0.076}\tableScoreSeparator\lIoU{0.051}\tableVerticalSeparator\\
&Self-Consistency~\cite{selfconsistency}&\bIoU{0.065}\tableScoreSeparator\sIoU{0.063} & \bIoU{\tbest{0.047}}\tableScoreSeparator\sIoU{0.047} & \bIoU{0.050}\tableScoreSeparator\sIoU{0.049} & \bIoU{0.047}\tableScoreSeparator\sIoU{0.046} & \bIoU{0.056}\tableScoreSeparator\sIoU{0.055} & \bIoU{0.055}\tableScoreSeparator\sIoU{0.054}\\
&with N-Cuts&\gIoU{0.066}\tableScoreSeparator\lIoU{0.074} & \gIoU{0.047}\tableScoreSeparator\lIoU{0.053} & \gIoU{0.050}\tableScoreSeparator\lIoU{0.056} & \gIoU{0.047}\tableScoreSeparator\lIoU{0.053} & \gIoU{0.057}\tableScoreSeparator\lIoU{0.063} & \gIoU{0.062}\tableScoreSeparator\lIoU{0.055}\tableVerticalSeparator\\
\bottomrule
\end{tabular}


==> table_f1.tex <==
%This file was automatically generated. Manual changes will be erased if the file is regenerated
\begin{tabular}{llcccccc}
\toprule
&&Noise&CFA Grid&CFA Algorithm&JPEG Grid&JPEG Quality&Hybrid\\\midrule
\multirow{8}{*}{\rotatebox{90}{Generic}}&\multirow{2}{*}{Noiseprint [15]}&\bIoU{0.163} & \bIoU{0.058} & \bIoU{0.106} & \bIoU{0.070} & \bIoU{0.234} & \bIoU{0.183}\\
&&\gIoU{0.207}\tableScoreSeparator\lIoU{0.283} & \gIoU{0.066}\tableScoreSeparator\lIoU{0.090} & \gIoU{0.131}\tableScoreSeparator\lIoU{0.192} & \gIoU{0.077}\tableScoreSeparator\lIoU{0.115} & \gIoU{0.263}\tableScoreSeparator\lIoU{0.342} & \gIoU{0.213}\tableScoreSeparator\lIoU{0.280}\tableVerticalSeparator\\
&\multirow{2}{*}{ManTraNet [44]}&\bIoU{0.098} & \bIoU{0.065} & \bIoU{0.135} & \bIoU{0.068} & \bIoU{0.207} & \bIoU{0.183}\\
&&\gIoU{0.110}\tableScoreSeparator\lIoU{0.141} & \gIoU{0.066}\tableScoreSeparator\lIoU{0.080} & \gIoU{0.137}\tableScoreSeparator\lIoU{0.190} & \gIoU{0.073}\tableScoreSeparator\lIoU{0.086} & \gIoU{0.220}\tableScoreSeparator\lIoU{0.286} & \gIoU{0.183}\tableScoreSeparator\lIoU{0.238}\tableVerticalSeparator\\
&\multirow{2}{*}{Self-Consistency [23]}&\bIoU{0.068} & \bIoU{0.058} & \bIoU{0.061} & \bIoU{0.059} & \bIoU{0.077} & \bIoU{0.067}\\
&&\gIoU{0.098}\tableScoreSeparator\lIoU{0.138} & \gIoU{0.068}\tableScoreSeparator\lIoU{0.096} & \gIoU{0.075}\tableScoreSeparator\lIoU{0.104} & \gIoU{0.067}\tableScoreSeparator\lIoU{0.094} & \gIoU{0.085}\tableScoreSeparator\lIoU{0.124} & \gIoU{0.083}\tableScoreSeparator\lIoU{0.120}\tableVerticalSeparator\\
&\multirow{2}{*}{Self-Consistency [23]nc}&\bIoU{0.095} & \bIoU{0.077} & \bIoU{0.080} & \bIoU{0.076} & \bIoU{0.085} & \bIoU{0.085}\\
&&\gIoU{0.096}\tableScoreSeparator\lIoU{0.107} & \gIoU{0.077}\tableScoreSeparator\lIoU{0.085} & \gIoU{0.080}\tableScoreSeparator\lIoU{0.088} & \gIoU{0.076}\tableScoreSeparator\lIoU{0.084} & \gIoU{0.086}\tableScoreSeparator\lIoU{0.094} & \gIoU{0.086}\tableScoreSeparator\lIoU{0.095}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{6}{*}{\rotatebox{90}{Noise}}&\multirow{2}{*}{Splicebuster [14]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.195}\tableScoreSeparator\lIoU{0.273} & \gIoU{0.073}\tableScoreSeparator\lIoU{0.104} & \gIoU{0.143}\tableScoreSeparator\lIoU{0.210} & \gIoU{0.071}\tableScoreSeparator\lIoU{0.104} & \gIoU{0.149}\tableScoreSeparator\lIoU{0.208} & \gIoU{0.160}\tableScoreSeparator\lIoU{0.219}\tableVerticalSeparator\\
&\multirow{2}{*}{Lyu [33]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.076}\tableScoreSeparator\lIoU{0.148} & \gIoU{0.063}\tableScoreSeparator\lIoU{0.085} & \gIoU{0.064}\tableScoreSeparator\lIoU{0.087} & \gIoU{0.063}\tableScoreSeparator\lIoU{0.084} & \gIoU{0.063}\tableScoreSeparator\lIoU{0.084} & \gIoU{0.064}\tableScoreSeparator\lIoU{0.104}\tableVerticalSeparator\\
&\multirow{2}{*}{Mahdian [34]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.095}\tableScoreSeparator\lIoU{0.266} & \gIoU{0.062}\tableScoreSeparator\lIoU{0.098} & \gIoU{0.072}\tableScoreSeparator\lIoU{0.151} & \gIoU{0.065}\tableScoreSeparator\lIoU{0.096} & \gIoU{0.070}\tableScoreSeparator\lIoU{0.135} & \gIoU{0.078}\tableScoreSeparator\lIoU{0.160}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{6}{*}{\rotatebox{90}{CFA}}&\multirow{2}{*}{Bammey [4]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.057}\tableScoreSeparator\lIoU{0.059} & \gIoU{0.604}\tableScoreSeparator\lIoU{0.618} & \gIoU{0.451}\tableScoreSeparator\lIoU{0.473} & \gIoU{0.058}\tableScoreSeparator\lIoU{0.066} & \gIoU{0.058}\tableScoreSeparator\lIoU{0.066} & \gIoU{0.126}\tableScoreSeparator\lIoU{0.144}\tableVerticalSeparator\\
&\multirow{2}{*}{Shin [40]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.063}\tableScoreSeparator\lIoU{0.070} & \gIoU{0.088}\tableScoreSeparator\lIoU{0.094} & \gIoU{0.080}\tableScoreSeparator\lIoU{0.089} & \gIoU{0.053}\tableScoreSeparator\lIoU{0.060} & \gIoU{0.053}\tableScoreSeparator\lIoU{0.060} & \gIoU{0.063}\tableScoreSeparator\lIoU{0.071}\tableVerticalSeparator\\
&\multirow{2}{*}{Choi [9]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.056}\tableScoreSeparator\lIoU{0.058} & \gIoU{0.056}\tableScoreSeparator\lIoU{0.059} & \gIoU{0.056}\tableScoreSeparator\lIoU{0.058} & \gIoU{0.056}\tableScoreSeparator\lIoU{0.059} & \gIoU{0.057}\tableScoreSeparator\lIoU{0.059} & \gIoU{0.056}\tableScoreSeparator\lIoU{0.058}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{14}{*}{\rotatebox{90}{JPEG}}&\multirow{2}{*}{Zero [37]}&\bIoU{0.052} & \bIoU{0.052} & \bIoU{0.052} & \bIoU{0.780} & \bIoU{0.762} & \bIoU{0.656}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue\tableVerticalSeparator\\
&\multirow{2}{*}{CAGI [24]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.091}\tableScoreSeparator\lIoU{0.184} & \gIoU{0.062}\tableScoreSeparator\lIoU{0.095} & \gIoU{0.068}\tableScoreSeparator\lIoU{0.118} & \gIoU{0.137}\tableScoreSeparator\lIoU{0.251} & \gIoU{0.139}\tableScoreSeparator\lIoU{0.255} & \gIoU{0.119}\tableScoreSeparator\lIoU{0.240}\tableVerticalSeparator\\
&\multirow{2}{*}{FDF-A [3]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.063}\tableScoreSeparator\lIoU{0.070} & \gIoU{0.056}\tableScoreSeparator\lIoU{0.061} & \gIoU{0.056}\tableScoreSeparator\lIoU{0.061} & \gIoU{0.173}\tableScoreSeparator\lIoU{0.184} & \gIoU{0.177}\tableScoreSeparator\lIoU{0.186} & \gIoU{0.162}\tableScoreSeparator\lIoU{0.172}\tableVerticalSeparator\\
&\multirow{2}{*}{I-CDA [5]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.053}\tableScoreSeparator\lIoU{0.053} & \gIoU{0.053}\tableScoreSeparator\lIoU{0.053} & \gIoU{0.053}\tableScoreSeparator\lIoU{0.053} & \gIoU{0.413}\tableScoreSeparator\lIoU{0.482} & \gIoU{0.400}\tableScoreSeparator\lIoU{0.468} & \gIoU{0.314}\tableScoreSeparator\lIoU{0.372}\tableVerticalSeparator\\
&\multirow{2}{*}{CDA [31]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.056}\tableScoreSeparator\lIoU{0.067} & \gIoU{0.055}\tableScoreSeparator\lIoU{0.067} & \gIoU{0.055}\tableScoreSeparator\lIoU{0.066} & \gIoU{0.354}\tableScoreSeparator\lIoU{0.397} & \gIoU{0.349}\tableScoreSeparator\lIoU{0.390} & \gIoU{0.296}\tableScoreSeparator\lIoU{0.339}\tableVerticalSeparator\\
&\multirow{2}{*}{BAG [29]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.052}\tableScoreSeparator\lIoU{0.053} & \gIoU{0.053}\tableScoreSeparator\lIoU{0.054} & \gIoU{0.054}\tableScoreSeparator\lIoU{0.054} & \gIoU{0.178}\tableScoreSeparator\lIoU{0.178} & \gIoU{0.178}\tableScoreSeparator\lIoU{0.178} & \gIoU{0.156}\tableScoreSeparator\lIoU{0.156}\tableVerticalSeparator\\
&\multirow{2}{*}{ELA [28]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.066}\tableScoreSeparator\lIoU{0.093} & \gIoU{0.058}\tableScoreSeparator\lIoU{0.065} & \gIoU{0.058}\tableScoreSeparator\lIoU{0.067} & \gIoU{0.095}\tableScoreSeparator\lIoU{0.119} & \gIoU{0.102}\tableScoreSeparator\lIoU{0.131} & \gIoU{0.099}\tableScoreSeparator\lIoU{0.128}\tableVerticalSeparator\\
\bottomrule
\end{tabular}

==> table_iou.tex <==
%This file was automatically generated. Manual changes will be erased if the file is regenerated
\begin{tabular}{llcccccc}
\toprule
&&Noise&CFA Grid&CFA Algorithm&JPEG Grid&JPEG Quality&Hybrid\\\midrule
\multirow{8}{*}{\rotatebox{90}{Generic}}&\multirow{2}{*}{Noiseprint [15]}&\bIoU{0.108}\tableScoreSeparator\sIoU{0.068} & \bIoU{0.034}\tableScoreSeparator\sIoU{0.033} & \bIoU{0.068}\tableScoreSeparator\sIoU{0.047} & \bIoU{0.042}\tableScoreSeparator\sIoU{0.034} & \bIoU{0.166}\tableScoreSeparator\sIoU{0.071} & \bIoU{0.127}\tableScoreSeparator\sIoU{0.065}\\
&&\gIoU{0.152}\tableScoreSeparator\lIoU{0.217} & \gIoU{0.039}\tableScoreSeparator\lIoU{0.054} & \gIoU{0.091}\tableScoreSeparator\lIoU{0.137} & \gIoU{0.047}\tableScoreSeparator\lIoU{0.071} & \gIoU{0.202}\tableScoreSeparator\lIoU{0.270} & \gIoU{0.159}\tableScoreSeparator\lIoU{0.217}\tableVerticalSeparator\\
&\multirow{2}{*}{ManTraNet [44]}&\bIoU{0.059}\tableScoreSeparator\sIoU{0.050} & \bIoU{0.038}\tableScoreSeparator\sIoU{0.036} & \bIoU{0.087}\tableScoreSeparator\sIoU{0.062} & \bIoU{0.040}\tableScoreSeparator\sIoU{0.036} & \bIoU{0.142}\tableScoreSeparator\sIoU{0.082} & \bIoU{0.124}\tableScoreSeparator\sIoU{0.078}\\
&&\gIoU{0.067}\tableScoreSeparator\lIoU{0.088} & \gIoU{0.039}\tableScoreSeparator\lIoU{0.047} & \gIoU{0.089}\tableScoreSeparator\lIoU{0.129} & \gIoU{0.042}\tableScoreSeparator\lIoU{0.050} & \gIoU{0.162}\tableScoreSeparator\lIoU{0.214} & \gIoU{0.125}\tableScoreSeparator\lIoU{0.169}\tableVerticalSeparator\\
&\multirow{2}{*}{Self-Consistency [23]}&\bIoU{0.042}\tableScoreSeparator\sIoU{0.041} & \bIoU{0.035}\tableScoreSeparator\sIoU{0.035} & \bIoU{0.037}\tableScoreSeparator\sIoU{0.035} & \bIoU{0.035}\tableScoreSeparator\sIoU{0.034} & \bIoU{0.048}\tableScoreSeparator\sIoU{0.037} & \bIoU{0.041}\tableScoreSeparator\sIoU{0.038}\\
&&\gIoU{0.064}\tableScoreSeparator\lIoU{0.092} & \gIoU{0.041}\tableScoreSeparator\lIoU{0.059} & \gIoU{0.046}\tableScoreSeparator\lIoU{0.066} & \gIoU{0.040}\tableScoreSeparator\lIoU{0.057} & \gIoU{0.054}\tableScoreSeparator\lIoU{0.082} & \gIoU{0.051}\tableScoreSeparator\lIoU{0.076}\tableVerticalSeparator\\
&\multirow{2}{*}{Self-Consistency [23]nc}&\bIoU{0.065}\tableScoreSeparator\sIoU{0.063} & \bIoU{0.047}\tableScoreSeparator\sIoU{0.047} & \bIoU{0.050}\tableScoreSeparator\sIoU{0.049} & \bIoU{0.047}\tableScoreSeparator\sIoU{0.046} & \bIoU{0.056}\tableScoreSeparator\sIoU{0.055} & \bIoU{0.055}\tableScoreSeparator\sIoU{0.054}\\
&&\gIoU{0.066}\tableScoreSeparator\lIoU{0.074} & \gIoU{0.047}\tableScoreSeparator\lIoU{0.053} & \gIoU{0.050}\tableScoreSeparator\lIoU{0.056} & \gIoU{0.047}\tableScoreSeparator\lIoU{0.053} & \gIoU{0.057}\tableScoreSeparator\lIoU{0.063} & \gIoU{0.055}\tableScoreSeparator\lIoU{0.062}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{6}{*}{\rotatebox{90}{Noise}}&\multirow{2}{*}{Splicebuster [14]}&\noTableValue\tableScoreSeparator\sIoU{0.073} & \noTableValue\tableScoreSeparator\sIoU{0.036} & \noTableValue\tableScoreSeparator\sIoU{0.056} & \noTableValue\tableScoreSeparator\sIoU{0.036} & \noTableValue\tableScoreSeparator\sIoU{0.059} & \noTableValue\tableScoreSeparator\sIoU{0.063}\\
&&\gIoU{0.139}\tableScoreSeparator\lIoU{0.203} & \gIoU{0.045}\tableScoreSeparator\lIoU{0.065} & \gIoU{0.097}\tableScoreSeparator\lIoU{0.149} & \gIoU{0.043}\tableScoreSeparator\lIoU{0.064} & \gIoU{0.104}\tableScoreSeparator\lIoU{0.148} & \gIoU{0.112}\tableScoreSeparator\lIoU{0.157}\tableVerticalSeparator\\
&\multirow{2}{*}{Lyu [33]}&\noTableValue\tableScoreSeparator\sIoU{0.035} & \noTableValue\tableScoreSeparator\sIoU{0.034} & \noTableValue\tableScoreSeparator\sIoU{0.035} & \noTableValue\tableScoreSeparator\sIoU{0.035} & \noTableValue\tableScoreSeparator\sIoU{0.035} & \noTableValue\tableScoreSeparator\sIoU{0.034}\\
&&\gIoU{0.046}\tableScoreSeparator\lIoU{0.096} & \gIoU{0.037}\tableScoreSeparator\lIoU{0.050} & \gIoU{0.038}\tableScoreSeparator\lIoU{0.052} & \gIoU{0.037}\tableScoreSeparator\lIoU{0.050} & \gIoU{0.037}\tableScoreSeparator\lIoU{0.050} & \gIoU{0.037}\tableScoreSeparator\lIoU{0.063}\tableVerticalSeparator\\
&\multirow{2}{*}{Mahdian [34]}&\noTableValue\tableScoreSeparator\sIoU{0.036} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.033}\\
&&\gIoU{0.063}\tableScoreSeparator\lIoU{0.192} & \gIoU{0.037}\tableScoreSeparator\lIoU{0.058} & \gIoU{0.044}\tableScoreSeparator\lIoU{0.098} & \gIoU{0.038}\tableScoreSeparator\lIoU{0.057} & \gIoU{0.042}\tableScoreSeparator\lIoU{0.085} & \gIoU{0.049}\tableScoreSeparator\lIoU{0.106}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{6}{*}{\rotatebox{90}{CFA}}&\multirow{2}{*}{Bammey [4]}&\noTableValue\tableScoreSeparator\sIoU{0.034} & \noTableValue\tableScoreSeparator\sIoU{0.416} & \noTableValue\tableScoreSeparator\sIoU{0.303} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.086}\\
&&\gIoU{0.034}\tableScoreSeparator\lIoU{0.035} & \gIoU{0.498}\tableScoreSeparator\lIoU{0.511} & \gIoU{0.359}\tableScoreSeparator\lIoU{0.380} & \gIoU{0.035}\tableScoreSeparator\lIoU{0.039} & \gIoU{0.034}\tableScoreSeparator\lIoU{0.039} & \gIoU{0.089}\tableScoreSeparator\lIoU{0.103}\tableVerticalSeparator\\
&\multirow{2}{*}{Shin [40]}&\noTableValue\tableScoreSeparator\sIoU{0.036} & \noTableValue\tableScoreSeparator\sIoU{0.043} & \noTableValue\tableScoreSeparator\sIoU{0.042} & \noTableValue\tableScoreSeparator\sIoU{0.029} & \noTableValue\tableScoreSeparator\sIoU{0.029} & \noTableValue\tableScoreSeparator\sIoU{0.034}\\
&&\gIoU{0.037}\tableScoreSeparator\lIoU{0.041} & \gIoU{0.054}\tableScoreSeparator\lIoU{0.058} & \gIoU{0.049}\tableScoreSeparator\lIoU{0.055} & \gIoU{0.031}\tableScoreSeparator\lIoU{0.035} & \gIoU{0.032}\tableScoreSeparator\lIoU{0.035} & \gIoU{0.038}\tableScoreSeparator\lIoU{0.042}\tableVerticalSeparator\\
&\multirow{2}{*}{Choi [9]}&\noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.033} & \noTableValue\tableScoreSeparator\sIoU{0.032}\\
&&\gIoU{0.033}\tableScoreSeparator\lIoU{0.034} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.035} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.034} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.035} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.035} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.034}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{14}{*}{\rotatebox{90}{JPEG}}&\multirow{2}{*}{Zero [37]}&\bIoU{0.031}\tableScoreSeparator\noTableValue & \bIoU{0.031}\tableScoreSeparator\noTableValue & \bIoU{0.031}\tableScoreSeparator\noTableValue & \bIoU{0.718}\tableScoreSeparator\noTableValue & \bIoU{0.700}\tableScoreSeparator\noTableValue & \bIoU{0.602}\tableScoreSeparator\noTableValue\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue\tableVerticalSeparator\\
&\multirow{2}{*}{CAGI [24]}&\noTableValue\tableScoreSeparator\sIoU{0.029} & \noTableValue\tableScoreSeparator\sIoU{0.028} & \noTableValue\tableScoreSeparator\sIoU{0.028} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.030}\\
&&\gIoU{0.061}\tableScoreSeparator\lIoU{0.131} & \gIoU{0.037}\tableScoreSeparator\lIoU{0.057} & \gIoU{0.041}\tableScoreSeparator\lIoU{0.075} & \gIoU{0.096}\tableScoreSeparator\lIoU{0.182} & \gIoU{0.097}\tableScoreSeparator\lIoU{0.187} & \gIoU{0.081}\tableScoreSeparator\lIoU{0.174}\tableVerticalSeparator\\
&\multirow{2}{*}{FDF-A [3]}&\noTableValue\tableScoreSeparator\sIoU{0.036} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.088} & \noTableValue\tableScoreSeparator\sIoU{0.091} & \noTableValue\tableScoreSeparator\sIoU{0.083}\\
&&\gIoU{0.037}\tableScoreSeparator\lIoU{0.042} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.036} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.036} & \gIoU{0.115}\tableScoreSeparator\lIoU{0.122} & \gIoU{0.118}\tableScoreSeparator\lIoU{0.124} & \gIoU{0.108}\tableScoreSeparator\lIoU{0.114}\tableVerticalSeparator\\
&\multirow{2}{*}{I-CDA [5]}&\noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.167} & \noTableValue\tableScoreSeparator\sIoU{0.160} & \noTableValue\tableScoreSeparator\sIoU{0.175}\\
&&\gIoU{0.031}\tableScoreSeparator\lIoU{0.031} & \gIoU{0.032}\tableScoreSeparator\lIoU{0.032} & \gIoU{0.032}\tableScoreSeparator\lIoU{0.032} & \gIoU{0.327}\tableScoreSeparator\lIoU{0.390} & \gIoU{0.317}\tableScoreSeparator\lIoU{0.378} & \gIoU{0.245}\tableScoreSeparator\lIoU{0.293}\tableVerticalSeparator\\
&\multirow{2}{*}{CDA [31]}&\noTableValue\tableScoreSeparator\sIoU{0.027} & \noTableValue\tableScoreSeparator\sIoU{0.027} & \noTableValue\tableScoreSeparator\sIoU{0.027} & \noTableValue\tableScoreSeparator\sIoU{0.217} & \noTableValue\tableScoreSeparator\sIoU{0.218} & \noTableValue\tableScoreSeparator\sIoU{0.187}\\
&&\gIoU{0.033}\tableScoreSeparator\lIoU{0.040} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.039} & \gIoU{0.033}\tableScoreSeparator\lIoU{0.039} & \gIoU{0.262}\tableScoreSeparator\lIoU{0.300} & \gIoU{0.260}\tableScoreSeparator\lIoU{0.297} & \gIoU{0.219}\tableScoreSeparator\lIoU{0.254}\tableVerticalSeparator\\
&\multirow{2}{*}{BAG [29]}&\noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.032} & \noTableValue\tableScoreSeparator\sIoU{0.127} & \noTableValue\tableScoreSeparator\sIoU{0.126} & \noTableValue\tableScoreSeparator\sIoU{0.109}\\
&&\gIoU{0.031}\tableScoreSeparator\lIoU{0.031} & \gIoU{0.032}\tableScoreSeparator\lIoU{0.032} & \gIoU{0.032}\tableScoreSeparator\lIoU{0.032} & \gIoU{0.128}\tableScoreSeparator\lIoU{0.128} & \gIoU{0.126}\tableScoreSeparator\lIoU{0.126} & \gIoU{0.109}\tableScoreSeparator\lIoU{0.109}\tableVerticalSeparator\\
&\multirow{2}{*}{ELA [28]}&\noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031} & \noTableValue\tableScoreSeparator\sIoU{0.031}\\
&&\gIoU{0.039}\tableScoreSeparator\lIoU{0.056} & \gIoU{0.034}\tableScoreSeparator\lIoU{0.038} & \gIoU{0.034}\tableScoreSeparator\lIoU{0.039} & \gIoU{0.056}\tableScoreSeparator\lIoU{0.071} & \gIoU{0.060}\tableScoreSeparator\lIoU{0.079} & \gIoU{0.059}\tableScoreSeparator\lIoU{0.077}\tableVerticalSeparator\\
\bottomrule
\end{tabular}

==> table_mcc.tex <==
%This file was automatically generated. Manual changes will be erased if the file is regenerated
\begin{tabular}{llcccccc}
\toprule
&&Noise&CFA Grid&CFA Algorithm&JPEG Grid&JPEG Quality&Hybrid\\\midrule
\multirow{8}{*}{\rotatebox{90}{Generic}}&\multirow{2}{*}{Noiseprint [15]}&\bIoU{0.160} & \bIoU{0.020} & \bIoU{0.081} & \bIoU{0.038} & \bIoU{0.228} & \bIoU{0.170}\\
&&\gIoU{0.209}\tableScoreSeparator\lIoU{0.283} & \gIoU{0.038}\tableScoreSeparator\lIoU{0.072} & \gIoU{0.115}\tableScoreSeparator\lIoU{0.180} & \gIoU{0.061}\tableScoreSeparator\lIoU{0.108} & \gIoU{0.264}\tableScoreSeparator\lIoU{0.347} & \gIoU{0.210}\tableScoreSeparator\lIoU{0.282}\tableVerticalSeparator\\
&\multirow{2}{*}{ManTraNet [44]}&\bIoU{0.073} & \bIoU{0.030} & \bIoU{0.120} & \bIoU{0.031} & \bIoU{0.194} & \bIoU{0.166}\\
&&\gIoU{0.102}\tableScoreSeparator\lIoU{0.127} & \gIoU{0.038}\tableScoreSeparator\lIoU{0.053} & \gIoU{0.120}\tableScoreSeparator\lIoU{0.170} & \gIoU{0.047}\tableScoreSeparator\lIoU{0.057} & \gIoU{0.200}\tableScoreSeparator\lIoU{0.264} & \gIoU{0.167}\tableScoreSeparator\lIoU{0.216}\tableVerticalSeparator\\
&\multirow{2}{*}{Self-Consistency [23]}&\bIoU{0.043} & \bIoU{0.024} & \bIoU{0.028} & \bIoU{0.028} & \bIoU{0.056} & \bIoU{0.036}\\
&&\gIoU{0.082}\tableScoreSeparator\lIoU{0.132} & \gIoU{0.043}\tableScoreSeparator\lIoU{0.088} & \gIoU{0.054}\tableScoreSeparator\lIoU{0.099} & \gIoU{0.042}\tableScoreSeparator\lIoU{0.091} & \gIoU{0.068}\tableScoreSeparator\lIoU{0.128} & \gIoU{0.064}\tableScoreSeparator\lIoU{0.114}\tableVerticalSeparator\\
&\multirow{2}{*}{Self-Consistency [23]nc}&\bIoU{0.112} & \bIoU{0.087} & \bIoU{0.091} & \bIoU{0.088} & \bIoU{0.101} & \bIoU{0.099}\\
&&\gIoU{0.112}\tableScoreSeparator\lIoU{0.128} & \gIoU{0.087}\tableScoreSeparator\lIoU{0.101} & \gIoU{0.091}\tableScoreSeparator\lIoU{0.106} & \gIoU{0.088}\tableScoreSeparator\lIoU{0.102} & \gIoU{0.101}\tableScoreSeparator\lIoU{0.115} & \gIoU{0.099}\tableScoreSeparator\lIoU{0.114}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{6}{*}{\rotatebox{90}{Noise}}&\multirow{2}{*}{Splicebuster [14]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.189}\tableScoreSeparator\lIoU{0.256} & \gIoU{0.046}\tableScoreSeparator\lIoU{0.080} & \gIoU{0.134}\tableScoreSeparator\lIoU{0.193} & \gIoU{0.044}\tableScoreSeparator\lIoU{0.079} & \gIoU{0.134}\tableScoreSeparator\lIoU{0.192} & \gIoU{0.143}\tableScoreSeparator\lIoU{0.197}\tableVerticalSeparator\\
&\multirow{2}{*}{Lyu [33]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.054}\tableScoreSeparator\lIoU{0.097} & \gIoU{0.046}\tableScoreSeparator\lIoU{0.063} & \gIoU{0.046}\tableScoreSeparator\lIoU{0.064} & \gIoU{0.045}\tableScoreSeparator\lIoU{0.063} & \gIoU{0.046}\tableScoreSeparator\lIoU{0.063} & \gIoU{0.043}\tableScoreSeparator\lIoU{0.075}\tableVerticalSeparator\\
&\multirow{2}{*}{Mahdian [34]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.092}\tableScoreSeparator\lIoU{0.245} & \noTableValue\tableScoreSeparator\noTableValue & \gIoU{0.043}\tableScoreSeparator\lIoU{0.130} & \gIoU{0.032}\tableScoreSeparator\lIoU{0.074} & \gIoU{0.039}\tableScoreSeparator\lIoU{0.109} & \gIoU{0.050}\tableScoreSeparator\lIoU{0.136}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{6}{*}{\rotatebox{90}{CFA}}&\multirow{2}{*}{Bammey [4]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.020}\tableScoreSeparator\lIoU{0.022} & \gIoU{0.603}\tableScoreSeparator\lIoU{0.616} & \gIoU{0.456}\tableScoreSeparator\lIoU{0.474} & \gIoU{0.036}\tableScoreSeparator\lIoU{0.048} & \gIoU{0.034}\tableScoreSeparator\lIoU{0.046} & \gIoU{0.109}\tableScoreSeparator\lIoU{0.128}\tableVerticalSeparator\\
&\multirow{2}{*}{Shin [40]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.042}\tableScoreSeparator\lIoU{0.050} & \gIoU{0.091}\tableScoreSeparator\lIoU{0.101} & \gIoU{0.078}\tableScoreSeparator\lIoU{0.092} & \gIoU{0.022}\tableScoreSeparator\lIoU{0.032} & \gIoU{0.022}\tableScoreSeparator\lIoU{0.031} & \gIoU{0.036}\tableScoreSeparator\lIoU{0.047}\tableVerticalSeparator\\
&\multirow{2}{*}{Choi [9]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.024}\tableScoreSeparator\lIoU{0.025} & \gIoU{0.024}\tableScoreSeparator\lIoU{0.026} & \gIoU{0.025}\tableScoreSeparator\lIoU{0.026} & \gIoU{0.024}\tableScoreSeparator\lIoU{0.026} & \gIoU{0.025}\tableScoreSeparator\lIoU{0.027} & \gIoU{0.024}\tableScoreSeparator\lIoU{0.026}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{14}{*}{\rotatebox{90}{JPEG}}&\multirow{2}{*}{Zero [37]}&\bIoU{0.000} & \bIoU{0.000} & \bIoU{0.000} & \bIoU{0.778} & \bIoU{0.758} & \bIoU{0.644}\\
&&\noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue & \noTableValue\tableScoreSeparator\noTableValue\tableVerticalSeparator\\
&\multirow{2}{*}{CAGI [24]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.072}\tableScoreSeparator\lIoU{0.166} & \gIoU{0.037}\tableScoreSeparator\lIoU{0.086} & \gIoU{0.046}\tableScoreSeparator\lIoU{0.107} & \gIoU{0.124}\tableScoreSeparator\lIoU{0.230} & \gIoU{0.129}\tableScoreSeparator\lIoU{0.236} & \gIoU{0.100}\tableScoreSeparator\lIoU{0.211}\tableVerticalSeparator\\
&\multirow{2}{*}{FDF-A [3]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.046}\tableScoreSeparator\lIoU{0.055} & \gIoU{0.032}\tableScoreSeparator\lIoU{0.040} & \gIoU{0.032}\tableScoreSeparator\lIoU{0.040} & \gIoU{0.177}\tableScoreSeparator\lIoU{0.183} & \gIoU{0.177}\tableScoreSeparator\lIoU{0.183} & \gIoU{0.161}\tableScoreSeparator\lIoU{0.168}\tableVerticalSeparator\\
&\multirow{2}{*}{I-CDA [5]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.006}\tableScoreSeparator\lIoU{0.006} & \gIoU{0.010}\tableScoreSeparator\lIoU{0.010} & \gIoU{0.013}\tableScoreSeparator\lIoU{0.013} & \gIoU{0.452}\tableScoreSeparator\lIoU{0.483} & \gIoU{0.438}\tableScoreSeparator\lIoU{0.469} & \gIoU{0.352}\tableScoreSeparator\lIoU{0.374}\tableVerticalSeparator\\
&\multirow{2}{*}{CDA [31]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.019}\tableScoreSeparator\lIoU{0.033} & \gIoU{0.018}\tableScoreSeparator\lIoU{0.032} & \gIoU{0.018}\tableScoreSeparator\lIoU{0.032} & \gIoU{0.387}\tableScoreSeparator\lIoU{0.403} & \gIoU{0.381}\tableScoreSeparator\lIoU{0.396} & \gIoU{0.328}\tableScoreSeparator\lIoU{0.344}\tableVerticalSeparator\\
&\multirow{2}{*}{BAG [29]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.006}\tableScoreSeparator\lIoU{0.006} & \gIoU{0.010}\tableScoreSeparator\lIoU{0.011} & \gIoU{0.014}\tableScoreSeparator\lIoU{0.014} & \gIoU{0.218}\tableScoreSeparator\lIoU{0.218} & \gIoU{0.215}\tableScoreSeparator\lIoU{0.215} & \gIoU{0.178}\tableScoreSeparator\lIoU{0.178}\tableVerticalSeparator\\
&\multirow{2}{*}{ELA [28]}&\noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue & \noTableValue\\
&&\gIoU{0.000}\tableScoreSeparator\lIoU{0.000} & \gIoU{0.000}\tableScoreSeparator\lIoU{0.000} & \gIoU{0.000}\tableScoreSeparator\lIoU{0.000} & \gIoU{0.000}\tableScoreSeparator\lIoU{0.000} & \gIoU{0.000}\tableScoreSeparator\lIoU{0.000} & \gIoU{0.000}\tableScoreSeparator\lIoU{0.000}\tableVerticalSeparator\\
\bottomrule
\end{tabular}

==> table_sv.tex <==
\begin{tabular}{llcccccc}
\toprule
&&&&Dataset\vspace{7pt}\\
&&Noise Level&CFA Grid&CFA Algorithm&JPEG Grid&JPEG Quality&Hybrid\\\midrule
\multirow{6}{*}{\rotatebox{90}{Noise-based}}&\multirow{2}{*}{Splicebuster~\cite{splicebuster2015}}&\ASEM{0.099}{0.188}&\NV&\NV&\NV&\ASEM{0.084}{0.175}&\ASEM{0.101}{0.192}\\
&&\SEM{0.100}{0.217}&\NV&\NV&\NV&\SEM{0.082}{0.220}&\SEM{0.099}{0.215}\tableVerticalSeparator\\
&\multirow{2}{*}{Lyu~\cite{lyupan2013}}&\ASEM{0.002}{0.103}&\NV&\NV&\NV&\NV&\ASEM{0.007}{0.109}\\
&&\SEM{-0.000}{0.154}&\NV&\NV&\NV&\SEM{0.007}{0.175}&\SEM{0.011}{0.167}\tableVerticalSeparator\\
&\multirow{2}{*}{Mahdian~\cite{mahdian2009}}&\ASEM{0.026}{0.168}&\NV&\NV&\NV&\ASEM{0.017}{0.158}&\ASEM{0.013}{0.189}\\
&&\SEM{0.034}{0.191}&\NV&\NV&\NV&\SEM{0.023}{0.218}&\SEM{0.026}{0.230}\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{6}{*}{\rotatebox{90}{CFA-based}}&\multirow{2}{*}{Bammey~\cite{bammey}}&\ASEM{0.007}{0.084}&\ASEM{0.682}{0.329}&\ASEM{0.501}{0.427}&\ASEM{0.023}{0.095}&\ASEM{0.029}{0.091}&\ASEM{0.133}{0.288}\\
&&\SEM{0.021}{0.153}&\SEM{0.665}{0.349}&\SEM{0.491}{0.429}&\SEM{0.018}{0.107}&\SEM{0.020}{0.100}&\SEM{0.128}{0.290}\tableVerticalSeparator\\
&\multirow{2}{*}{Shin~\cite{shin2017color}}&\NV&\NV&\NV&\NV&\NV&\NV\\
&&\NV&\NV&\NV&\NV&\NV&\NV\tableVerticalSeparator\\
&\multirow{2}{*}{Choi~\cite{choi}}&\NV&\NV&\NV&\NV&\NV&\NV\\
&&\NV&\NV&\NV&\NV&\NV&\NV\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{10}{*}{\rotatebox{90}{JPEG-based}}&\multirow{2}{*}{Zero~\cite{ZERO}}&\ASEM{0.000}{0.000}&\ASEM{0.000}{0.000}&\ASEM{0.000}{0.000}&\ASEM{0.796}{0.349}&\ASEM{0.732}{0.413}&\ASEM{0.638}{0.451}\\
&&\SEM{0.000}{0.000}&\SEM{0.000}{0.000}&\SEM{0.000}{0.000}&\SEM{0.756}{0.387}&\SEM{0.708}{0.421}&\SEM{0.624}{0.453}\tableVerticalSeparator\\
&\multirow{2}{*}{FDF-A~\cite{ADQ3}}&\multirow{2}{*}{\NV}&\NV&\NV&\NV&\NV&\NV\\
&&&\NV&\NV&\NV&\NV&\NV\tableVerticalSeparator\\
&\multirow{2}{*}{CAGI~\cite{CAGI}}&\ASEM{0.004}{0.045}&\NV&\NV&\ASEM{0.038}{0.077}&\ASEM{0.044}{0.080}&\ASEM{0.031}{0.071}\\
&&\SEM{0.003}{0.052}&\NV&\NV&\SEM{0.023}{0.077}&\SEM{0.028}{0.082}&\SEM{0.021}{0.073}\tableVerticalSeparator\\
&\multirow{2}{*}{I-CDA~\cite{ADQ2}}&\NV&\NV&\NV&\ASEM{0.415}{0.417}&\ASEM{0.422}{0.407}&\NV\\
&&\NV&\NV&\NV&\SEM{0.422}{0.408}&\SEM{0.413}{0.414}&\NV\tableVerticalSeparator\\
&\multirow{2}{*}{CDA~\cite{ADQ1}}&\NV&\NV&\NV&\ASEM{0.485}{0.339}&\ASEM{0.473}{0.344}&\NV\\
&&\NV&\NV&\NV&\SEM{0.448}{0.351}&\SEM{0.441}{0.350}&\NV\tableVerticalSeparator\\
&\multirow{2}{*}{BAG~\cite{BLK}}&\NV&\NV&\NV&\ASEM{0.231}{0.461}&\ASEM{0.228}{0.458}&\NV\\
&&\NV&\NV&\NV&\SEM{0.226}{0.459}&\SEM{0.222}{0.455}&\NV\tableVerticalSeparator\\
\cmidrule{1-2}
\multirow{6}{*}{\rotatebox{90}{Generic tools}}&\multirow{2}{*}{\multirow{2}{*}{Noiseprint~\cite{noiseprint}}}&\ASEM{0.109}{0.181}&\ASEM{0.013}{0.074}&\ASEM{0.057}{0.141}&\ASEM{0.015}{0.086}&\ASEM{0.192}{0.224}&\ASEM{0.169}{0.228}\\
&&\SEM{0.108}{0.232}&\SEM{0.002}{0.114}&\SEM{0.060}{0.179}&\SEM{0.016}{0.140}&\SEM{0.138}{0.279}&\SEM{0.128}{0.261}\tableVerticalSeparator\\
&\multirow{2}{*}{\multirow{2}{*}{ManTraNet~\cite{mantranet}}}&\ASEM{0.056}{0.089}&\ASEM{0.007}{0.043}&\ASEM{0.072}{0.158}&\ASEM{0.007}{0.022}&\ASEM{0.097}{0.155}&\ASEM{0.107}{0.162}\\
&&\SEM{0.033}{0.100}&\SEM{-0.002}{0.071}&\SEM{0.056}{0.164}&\SEM{0.002}{0.042}&\SEM{0.082}{0.157}&\SEM{0.094}{0.160}\tableVerticalSeparator\\
%&\multirow{2}{*}{Self-Consistency~\cite{selfconsistency}}&\ASEM{0.041}{0.147}&\ASEM{0.008}{0.113}&\ASEM{0.016}{0.123}&\ASEM{-0.000}{0.099}&\ASEM{0.041}{0.133}&\ASEM{0.079}{0.172}\\
%&&\SEM{0.088}{0.222}&\SEM{0.039}{0.187}&\SEM{0.043}{0.198}&\SEM{0.035}{0.171}&\SEM{0.081}{0.208}&\SEM{0.119}{0.224}\tableVerticalSeparator\\
&Self-&\ASEM{0.056}{0.310}&\ASEM{0.018}{0.254}&\ASEM{0.020}{0.263}&\ASEM{-0.014}{0.250}&\ASEM{0.062}{0.329}&\ASEM{0.123}{0.366}\\
&-Consistency~\cite{selfconsistency}&\SEM{0.146}{0.422}&\SEM{0.072}{0.385}&\SEM{0.079}{0.397}&\SEM{0.047}{0.376}&\SEM{0.139}{0.432}&\SEM{0.239}{0.423}\tableVerticalSeparator\\
\bottomrule
\end{tabular}


==> visual_results_old.tex <==
\def\s{0.11\textwidth}
\begin{tabular}{lcccccc}
%\toprule
&Noise Level&CFA Grid&CFA Algorithm&JPEG Grid&JPEG Quality&Hybrid\\

%\multirow{2}{*}&& $1.8482320142031017$ $5.621304583865482 $ & GRBG  & BGGR AAHD & 97 & 96 & Noise 1.6086415606968902 2.2789071071428477 0.5339502978989161 2.840742885821646\\
%$0.5021874771955884$ $0.2874773899084025 $ & &  & 2 3 & 93 7 3 & JPEGQual 93 75 1 0 CFAAlg GRBG DCB\\
%\midrule

\raisebox{16pt}{Splicebuster~\cite{splicebuster2015}}
&\includegraphics[width=\s]{figures/example/sb_noise.png}
&\raisebox{16pt}{---}%\includegraphics[width=\s]{figures/example/cfa_grid/splicebuster_h.png} 
&\includegraphics[width=\s]{figures/example/sb_cfa_alg.png} 
&\raisebox{16pt}{---}%\includegraphics[width=\s]{figures/example/jpeg_grid/splicebuster_h.png} 
&\includegraphics[width=\s]{figures/example/sb_jpeg_quality.png} 
&\includegraphics[width=\s]{figures/example/sb_hybrid_select.png} \\

\raisebox{16pt}{Bammey~\cite{bammey}}
&\raisebox{16pt}{---}%\includegraphics[width=\s]{figures/example/noise/bammey20_b32_h.png}
&\includegraphics[width=\s]{figures/example/cfa_grid/bammey20_b32_h.png} 
&\includegraphics[width=\s]{figures/example/cfa_algorithm/bammey20_b32_h.png} 
&\raisebox{16pt}{---}%\includegraphics[width=\s]{figures/example/jpeg_grid/bammey20_b32_h.png} 
&\raisebox{16pt}{---}%\includegraphics[width=\s]{figures/example/jpeg_quality/bammey20_b32_h.png} 
&\includegraphics[width=\s]{figures/example/hybrid_select/bammey20_b32_h.png} \\

\raisebox{16pt}{ZERO~\cite{ZERO}}
&\raisebox{16pt}{---}%\includegraphics[width=\s]{figures/example/noise/zero_b.png}
&\raisebox{16pt}{---}%\includegraphics[width=\s]{figures/example/cfa_grid/zero_b.png} 
&\raisebox{16pt}{---}%\includegraphics[width=\s]{figures/example/cfa_algorithm/zero_b.png} 
&\includegraphics[width=\s]{figures/example/jpeg_grid/zero_b.png} 
&\includegraphics[width=\s]{figures/example/jpeg_quality/zero_b.png} 
&\includegraphics[width=\s]{figures/example/hybrid_select/zero_b.png} \\

\raisebox{16pt}{Noiseprint~\cite{noiseprint}}
&\includegraphics[width=\s]{figures/example/noise/noiseprint_h.png}
&\includegraphics[width=\s]{figures/example/cfa_grid/noiseprint_h.png} 
&\includegraphics[width=\s]{figures/example/cfa_algorithm/noiseprint_h.png} 
&\includegraphics[width=\s]{figures/example/jpeg_grid/noiseprint_h.png} 
&\includegraphics[width=\s]{figures/example/jpeg_quality/noiseprint_h.png} 
&\includegraphics[width=\s]{figures/example/hybrid_select/noiseprint_h.png} \\

\raisebox{16pt}{ManTraNet~\cite{mantranet}}
&\includegraphics[width=\s]{figures/example/noise/mantranet_h.png}
&\includegraphics[width=\s]{figures/example/cfa_grid/mantranet_h.png} 
&\includegraphics[width=\s]{figures/example/cfa_algorithm/mantranet_h.png} 
&\includegraphics[width=\s]{figures/example/jpeg_grid/mantranet_h.png} 
&\includegraphics[width=\s]{figures/example/jpeg_quality/mantranet_h.png} 
&\includegraphics[width=\s]{figures/example/hybrid_select/mantranet_h.png} \\

\raisebox{16pt}{Self-Consistency~\cite{selfconsistency}}
&\includegraphics[width=\s]{figures/example/noise/selfconsistency_ncuts_h.png}
&\includegraphics[width=\s]{figures/example/cfa_grid/selfconsistency_ncuts_h.png} 
&\includegraphics[width=\s]{figures/example/cfa_algorithm/selfconsistency_ncuts_h.png} 
&\includegraphics[width=\s]{figures/example/jpeg_grid/selfconsistency_ncuts_h.png} 
&\includegraphics[width=\s]{figures/example/jpeg_quality/selfconsistency_ncuts_h.png} 
&\includegraphics[width=\s]{figures/example/hybrid_select/selfconsistency_ncuts_h.png} \\
% \midrule
% \raisebox{16pt}{Ground Truth}
% &\includegraphics[width=\s]{figures/example/mask.png}
% &\includegraphics[width=\s]{figures/example/mask.png}
% &\includegraphics[width=\s]{figures/example/mask.png}
% &\includegraphics[width=\s]{figures/example/mask.png}
% &\includegraphics[width=\s]{figures/example/mask.png}
% &\includegraphics[width=\s]{figures/example/mask.png}\\
%\bottomrule

\end{tabular}
